Fast decision tree learning solves hard coding-theoretic problems

We connect the problem of properly PAC learning decision trees to the parameterized Nearest Codeword Problem ($k$-NCP). Despite significant effort by the respective communities, algorithmic progress on both problems has been stuck: the fastest known algorithm for the former runs in quasipolynomial time (Ehrenfeucht and Haussler 1989) and the best known approximation ratio for the latter is $O(n/\log n)$ (Berman and Karpinsky 2002; Alon, Panigrahy, and Yekhanin 2009). Research on both problems has thus far proceeded independently with no known connections. We show that $\textit{any}$ improvement of Ehrenfeucht and Haussler's algorithm will yield $O(\log n)$-approximation algorithms for $k$-NCP, an exponential improvement of the current state of the art. This can be interpreted either as a new avenue for designing algorithms for $k$-NCP, or as one for establishing the optimality of Ehrenfeucht and Haussler's algorithm. Furthermore, our reduction along with existing inapproximability results for $k$-NCP already rule out polynomial-time algorithms for properly learning decision trees. A notable aspect of our hardness results is that they hold even in the setting of $\textit{weak}$ learning whereas prior ones were limited to the setting of strong learning.

==> dt-learn.tex <==



\section{Implications for decision tree learning}
\label{sec:dt-learn}
\red{This section is old and needs to be incorporated into the body}
%\lnote{Restructure this section as follows: 
%\begin{enumerate}
%\item Move all the parameterized complexity of NCP stuff to the preliminaries,~\Cref{sec:hardness of NCP}. 
%\item Introduce the problem of decision tree learning 
%\item State the EH algorithm and its guarantees 
%\item State our sequence of 3 results that together suggest the optimality of EH even in the setting of weak learning.
%\item Sections for proofs 
%\end{enumerate}
%}

\subsection{$\mathrm{W}[1]$-hardness of decision tree learning: Proof of \Cref{thm:weak learning DTs}}

% The formal theorem we prove in this section is the following.
% \begin{theorem}[{${\mathrm{W}[1]}$-hardness of properly weak learning decision trees}] \lnote{This looks basically identical to~\Cref{thm:weak learning DTs}. If so, delete. }
% \label{thm:W[1] weak learning formal}
%     Assuming randomized $\mathrm{W}[1]\neq\mathrm{FPT}$, there is no algorithm running in $\poly(n)$ time which solves {\sc DT-Learn$(n,-,\eps)$} with $\eps=\frac{1}{2}-\frac{1}{\poly(n)}$.
%     % For all $c>0$, the following task is $\mathrm{W}[1]$-hard under a randomized polynomial-time reduction. Given random samples from a distribution $\mathcal{D}$ labeled by a unknown size-$n$ decision tree $T^\star:\zo^n\to\zo$, output in polynomial-time a decision tree $T_{\mathrm{hyp}}$ satisfying $\dist_{\mathcal{D}}(T^\star,T_{\mathrm{hyp}})\le \frac{1}{2}-\frac{1}{n^c}$.
%     % Assuming $\mathrm{W}[1] \ne \mathrm{FPT}$, there is no distribution-free algorithm for properly weak learning size-$s$ decision trees over $n$-variables in time $\poly(s,n)$ for $s=n$.
% \end{theorem}

To prove this theorem, we give a randomized FPT-reduction from constant-factor approximating NCP to weak learning decision trees.

    Let $\mathcal{A}$ be the decision tree learning algorithm from the theorem statement. Let $c>1$ be a large enough constant such that $\mathcal{A}$ runs in time $(s\cdot n)^c$ and with high probability outputs a decision tree $T_{\mathrm{hyp}}$ satisfying $\dist_{\mathcal{D}}(T^\star,T_{\mathrm{hyp}})\le \frac{1}{2}-\frac{1}{n^c}$ when run on an unknown size-$s$ decision tree $T^\star:\zo^n\to\zo$ and distribution $\mathcal{D}$. Using $\mathcal{A}$, we will solve $c'$-approximate $k$-NCP in $\poly(n)$ time for some large constant $c'>c$.

    \paragraph{The reduction.}{
        Let $(H,t)\in\F_2^{m\times n}\times\F_2^m$ be an instance of $c'$-approximate $k$-NCP where $H$ is the parity check matrix for the code $\mathcal{C}$. Assume $n$ is large enough so that $\log n\ge k$. Using \Cref{thm:general main reduction} with $\ell=\frac{\log n}{k}$, we obtain a function $f^\star:\zo^{n\ell}\to\zo$ and a distribution $\mathcal{D}^\star$ over $\zo^{n\ell}$. Note that the number of variables of $f^\star$ is $n\ell\le n\log n$. 
        
        % Let $D=\{y^{(1)},\ldots,y^{(m)}\}\sse \F_2^n$ be the set corresponding to the rows of the parity check matrix $H$ and $f:D\to\F_2$ be the function labeling the set according to $s$, $f(y^{(i)})=s_i$. Let $\mathcal{D}$ be the distribution $\mathrm{Uniform}(\mathrm{Span}(D))$. Let $f^{\mathrm{ext}}:\textsc{Span}(D)\to\F_2$ be the extension of $f$ to $\textsc{Span}(D)$. Assume $n$ is large enough so that $\log n\ge k$. We prove the theorem for the function $f^\star=((f^{\mathrm{ext}})^{\oplus\ell})_{\oplus 2}:(\F_2^{2n})^\ell\to\F_2$ and the distribution $\mathcal{D}^\star=(\mathcal{D}^{\otimes \ell})_{\oplus 2}$ where $\ell\coloneqq \frac{\log n}{2k}$. Note that the number of variables of $f^\star$ is $2n\ell\le n\log n$. 

        We run the algorithm $\mathcal{A}$ on $f^\star$ and $\mathcal{D}^\star$ for $(2^{k\ell}\cdot (n\ell))^c\le n^{3c}$ time steps. Let $T_{\mathrm{hyp}}$ be the decision tree learned by $\mathcal{A}$. We compute an estimate, $\overline{\varepsilon}$, of the quantity $\dist_{\mathcal{D}^\star}(f^\star,T_{\mathrm{hyp}})$ in $\poly(n)$-time using $\poly(n)$ random samples from $\mathcal{D}^\star$ so that our estimate is, with high probability, within a factor of $\pm {n^{-3c}}$ of the true value. We return ``Yes'' if $\overline{\varepsilon}\le \frac{1}{2}-{n^{-2c}}+{n^{-3c}}$ and ``No'' otherwise. 
    
        % We assume $n$ is large enough so that $\log n\ge k$. Let $f:\F_2^{2n}\to\F_2$ and $\mathcal{D}$ be the function and distribution from \Cref{thm:main reduction} which satisfies (3') in the No case of NCP. We run algorithm $\mathcal{A}$ on $(f^{\oplus \ell})_{\oplus 2}:(\F_2^{O(n)})^\ell\to\F_2$ and $(\mathcal{D}^{\otimes\ell})_{\oplus 2}$ for $\ell\coloneqq \frac{\log n}{2k}$ and stop $\mathcal{A}$ after $(O(n^2)\cdot \ell)^c$ many time steps. Let $T$ be the decision tree learned by $\mathcal{A}$. 
    }

    \paragraph{Runtime.}{
        Both queries to $f^\star$ and random samples from $\mathcal{D}^\star$ can be supported in polynomial-time. We simulate $\mathcal{A}$ for $\poly(n)$ time steps, so the overall runtime of our reduction is $\poly(n)$. 
    }
    
    \paragraph{Correctness.}{
        To prove correctness, we show that if $(H,t)$ is a Yes instance of $c'$-approximate $k$-NCP, then we output Yes with high probability, and otherwise if $(H,t)$ is a No instance then our algorithm outputs No with high probability.\bigskip

{\bf Yes case: there is a $k$ sparse vector $x$ such that $Hx=t$.} In this case, $f^\star$ is a parity of at most $k\ell=\log n$ variables under $\mathcal{D}^\star$ by \Cref{thm:general main reduction}. Therefore, $f^\star$ is a decision tree of size $2^{\log n}=n$ under $\mathcal{D}^\star$. By running $\mathcal{A}$ for $(n\cdot 2n\ell)^c=(2^{k\ell}\cdot(2n\ell))^c\le n^{3c}$ time steps, we obtain a decision tree $T_{\mathrm{hyp}}$ which satisfies
        \begin{align*}
            \dist_{\mathcal{D}^\star}(f^\star,T_{\mathrm{hyp}})&\le \frac{1}{2}-\frac{1}{(n\ell)^c}\tag{Assumption on $\mathcal{A}$}\\
            &\le \frac{1}{2}-\frac{1}{n^{2c}}.\tag{$n\ell\le n^2$}
        \end{align*}
        Finally, with high probability, our estimate $\overline{\varepsilon}$ satisfies $$\overline{\varepsilon}\le \dist_{\mathcal{D}^\star}(f^\star,T_{\mathrm{hyp}})+\frac{1}{n^{3c}}\le \frac{1}{2}-\frac{1}{n^{2c}}+\frac{1}{n^{3c}}$$
        which ensures that our algorithm for NCP correctly outputs ``Yes.''\bigskip 
        
 {\bf No case: $Hx\neq t$ for all vectors $x$ of sparsity at most $c'k$.} The runtime of the learning algorithm $\mathcal{A}$ serves as an upper bound on the size of the decision tree hypothesis $T_{\mathrm{hyp}}$. Therefore, it is sufficient to show that in this case, any decision tree of size $n^{3c}$ must have large enough error so that our estimate $\overline{\eps}$ satisfies $\overline{\varepsilon}>\frac{1}{2}-{n^{-2c}}+{n^{-3c}}$ with high probability.
    
        % By \Cref{lem:boosting}, $f^{\mathrm{ext}}$ is $\frac1{2}$-far under $\mathcal{D}$ from every parity of at most $c'\cdot k$ variables. Therefore, by \Cref{cor:outer-parity}, $(f^{\mathrm{ext}})^{\oplus \ell}$ is $\frac{1}{2}$-far under $\mathcal{D}^{\otimes\ell}$ from every function of Fourier degree at most $c'k\ell$. Finally, \Cref{lem:parity-substitution-technical} implies that $((f^{\mathrm{ext}})^{\oplus \ell})_{\oplus 2}$ is $\frac{1}{2}-2^{-\Theta(c'k\ell)}$ far under $\mathcal{D}^\star=(\mathcal{D}^{\otimes \ell})_{\oplus 2}$ from every decision tree of size $2^{\Theta(c'k\ell)}$. 
        \Cref{thm:general main reduction} implies that $f^{\star}$ is $\frac{1}{2}-2^{-\Theta(c'k\ell)}$ far under $\mathcal{D}^\star$ from every decision tree of size $2^{\Theta(c'k\ell)}$. By choosing $c'$ sufficiently larger than $c$ (e.g.~by inspecting the parameters in \Cref{lem:parity-substitution-technical}, $c'=50c$ is more than sufficient), we have $2^{\Theta(c'k\ell)}=n^{\Theta(c')}>n^{3c}$ and $2^{-\Theta(c'k\ell)}=n^{-\Theta(c')}<n^{-2c}-2n^{-3c}$. This implies that any decision tree $T_{\mathrm{hyp}}$ of size at most $n^{3c}$ will have error at least $\dist_{\mathcal{D}^\star}(T_{\mathrm{hyp}},f^\star)> \frac{1}{2}-n^{-2c}+2n^{-3c}$. Therefore, our estimate $\overline{\eps}$ of $\dist_{\mathcal{D}^\star}(T_{\mathrm{hyp}},f^\star)$ will satisfy
        \begin{align*}
            \overline{\eps}&\ge \dist_{\mathcal{D}^\star}(T_{\mathrm{hyp}},f^\star)-\frac{1}{n^{3c}}\tag{Accuracy of $\overline{\varepsilon}$}\\
            &> \frac{1}{2}-\frac{1}{n^{2c}}+\frac{2}{n^{3c}}-\frac{1}{n^{3c}}\tag{$|T_{\mathrm{hyp}}|\le n^{3c}$}\\
            &=\frac{1}{2}-\frac{1}{n^{2c}}+\frac{1}{n^{3c}}
        \end{align*}
        with high probability. This ensures that our algorithm correctly outputs ``No''.}\hfill\qed

\subsection{Gap-ETH hardness of decision tree learning}
\Cref{thm:gap-eth-hardness} from \cite{Man20} is proved by the following reduction which will be useful for us. The reduction is implicit in \cite{Man20} by stringing together the reduction from 3-SAT to {\sc Label Cover} (\cite[Theorem 9]{Man20}), and from {\sc Label Cover} to NCP (\cite[Corollary 5]{Man20}).

\begin{theorem}[Reduction from 3-SAT to $k$-NCP]
\label{thm:manurangsi reduction}
    For all constants $c>1$ and $\lambda>0$, and for every $k\in\N$, there is a reduction running in time $\poly(k,m,2^{m/k})$ which maps 3-\textnormal{SAT} instances $\varphi$ consisting of $m$ clauses to \textnormal{NCP} instances $(G,z)$ of size $\poly(k,m,2^{m/k})$ such that 
    \begin{itemize}
        \item[$\circ$] \textnormal{Yes} case: if $\varphi$ is satisfiable then $(G,z)$ is a \textnormal{Yes} instance of $c$-approximate $k$-\textnormal{NCP}
        \item[$\circ$] \textnormal{No} case: if every assignment to $\varphi$ satisfies at most $(1-\lambda)m$ clauses, then $(G,z)$ is a \textnormal{No} instance of $c$-approximate $k$-\textnormal{NCP}.
    \end{itemize}
\end{theorem}


\begin{theorem}[Gap-ETH hardness of properly weak learning decision trees]
\label{thm:gap-eth weak learning formal}
    Assuming randomized \textnormal{Gap-ETH}, there is no algorithm running in time $n^{o(\log n)}$ for {\sc DT-Learn$(n,\poly(n),\eps)$} where $\eps=\frac{1}{2}-\frac{1}{\poly(n)}$.
    % the following task. Given random samples from a distribution $\mathcal{D}$ labeled by an unknown size-$n$ decision tree $T^\star:\zo^n\to\zo$, output in time $n^{o(\log n)}$ a decision tree $T_{\mathrm{hyp}}$ of size $\poly(n)$ satisfying $\dist_{\mathcal{D}}(T^\star,T_{\mathrm{hyp}})\le \frac{1}{2}-\frac{1}{n^c}$. 
\end{theorem}

The proof of \Cref{thm:gap-eth weak learning formal} follows the same high level approach as \Cref{thm:w1-hardness}. 

\begin{proof}
    Assume for contradiction there is an algorithm $\mathcal{A}$ solving the task in the theorem statement. Let $c>0$ be a large enough constant so that $\mathcal{A}$ outputs a decision tree $T_{\mathrm{hyp}}$ of size $n^c$ satisfying $\dist_{\mathcal{D}}(T^\star,T_{\mathrm{hyp}})\le\frac{1}{2}-\frac{1}{n^c}$ in time $n^{o(\log n)}$. Using $\mathcal{A}$, we will solve gapped 3-SAT in randomized time $2^{o(n)}$ for a given gap parameter $\delta>0$ thereby refuting randomized Gap-ETH.
    % $(k,c'\cdot k)$-NCP in time $n^{o(k)}$ for some large constant $c'>c$.

    \paragraph{The reduction.}{
        Let $\varphi$ be a 3-SAT instance on $n$ variables and with $m$ clauses and let $\delta>0$ be given. Using \Cref{thm:manurangsi reduction} with $k=\sqrt{m}$, we obtain a $c'$-approximate $k$-NCP instance $(H,t)\in\F_2^{M\times N}\times\F_2^M$ where $H$ is the parity check matrix for a linear code and $M+N=\poly(k,m,2^{O(m/k)})=2^{O(\sqrt{m})}$. Note in particular we can assume $2^{2k}\le 2N$ (this will satisfy our assumption on the size of the target decision tree). By \Cref{thm:manurangsi reduction}, to approximate the number of satisfiable clauses of $\varphi$, it is sufficient to solve $c'$-approximate $k$-NCP on $(H,t)$ in time $2^{o(m)}$. 
        
        Using \Cref{thm:general main reduction} with $\ell=2$, we obtain a function $f^\star:\zo^{2N}\to\zo$ and a distribution $\mathcal{D}^\star$ over $\zo^{2N}$. We run $\mathcal{A}$ on $f^\star$ and $\mathcal{D}^\star$ for $N^{o(\log N)}$ time steps. The algorithm outputs a decision tree $T_{\mathrm{hyp}}$. We estimate the quantity $\dist_{\mathcal{D}^\star}(T_{\mathrm{hyp}},f^\star)$ to accuracy $\pm \frac{1}{\poly(N)}$ in polynomial time using random samples from $\mathcal{D}^\star$. We return ``Yes'' if $\dist_{\mathcal{D}^\star}(f^\star,T_{\mathrm{hyp}})\le \frac{1}{2}-\frac{1}{(2N)^c}$ and $|T_{\mathrm{hyp}}|\le 2^{2ck}$, and ``No'' otherwise.
    }

    \paragraph{Runtime.}{
        Both queries to $f^\star$ and random samples from $\mathcal{D}^\star$ can be supported in polynomial-time. We simulate $\mathcal{A}$ for $\poly(N)$ time steps, so the overall runtime of our reduction is dominated by $N^{o(\log N)}$. In terms of the size of $\varphi$, the runtime is $(2^{O(\sqrt{m})})^{o(\sqrt{m})}=2^{o(m)}$ which is sufficient to refute Gap-ETH.
    }

    \paragraph{Correctness.}{We prove the yes and no case separately. Since this analysis is very similar to that in the proof of \Cref{thm:w1-hardness}, we omit redundant details.\bigskip
    
         {\bf Yes case: there is a $k$ sparse vector $x$ such that $Hx=t$.} In this case, $f^\star$ is a parity of at most $2k$ variables under $\mathcal{D}^\star$ by \Cref{thm:general main reduction}. Therefore, $f^\star$ is a decision tree of size $2^{2k}$ under $\mathcal{D}^\star$. By our assumption on $\mathcal{A}$, it returns a decision tree $T_{\mathrm{hyp}}$ of size $2^{2ck}$ in $N^{o(\log N)}$ time which satisfies $\dist_{\mathcal{D}^\star}(f^\star,T_{\mathrm{hyp}})\le \frac{1}{2}-\frac{1}{(2N)^c}$ with high probability. Therefore, our algorithm for NCP correctly outputs ``Yes'' with high probability.\bigskip

         {\bf No case: $Hx\neq t$ for all vectors $x$ of sparsity at most $c'k$.} Our algorithm correctly outputs ``No'' if $|T_{\mathrm{hyp}}|>2^{2ck}$. Otherwise, assume that $|T_{\mathrm{hyp}}|\le 2^{2ck}$. We will show that $\dist_{\mathcal{D}^\star}(f^\star,T_{\mathrm{hyp}})>\frac{1}{2}-\frac{1}{(2N)^c}$ so that in this case our algorithm also correctly outputs ``No''. By \Cref{thm:general main reduction}, $f^\star$ is $\frac{1}{2}-2^{-\Theta(c'k)}=\frac{1}{2}-N^{-\Theta(c')}$ far under $\mathcal{D}^\star$ from every decision tree of size $2^{\Theta(c'k)}=N^{\Theta(c')}$. Therefore, choosing $c'$ large enough this ensures that any decision tree of size at most $2^{2ck}\le N^{\Theta(c')}$ is $\frac{1}{2}-N^{-\Theta(c')}\ge \frac{1}{2}-\frac{1}{(2N)^c}$ far under $\mathcal{D}^\star$.
    }
\end{proof}

\subsection{Optimal hardness of decision tree learning under parameterized intractability of NCP: Proof of \Cref{thm: EH optimality intro}}

% \lnote{Sync up with and reference informal statement (\Cref{thm: EH optimality intro}) in the intro.}

\begin{theorem}[Formal version of \Cref{thm: EH optimality intro}]
\label{thm:EH optimality}
    If there is an algorithm running in time $n^{o(\log s)}$ for {\sc DT-Learn$(s,-,\eps)$} with $\eps=\frac{1}{2}-\frac{1}{\poly(n)}$, then there is an algorithm running in time $n^{o(k)}$ which solves $O(\log n)$-approximate\footnote{The constant hidden in the $O(\log n)$ factor depends only on the polynomial factor in $\eps=\frac{1}{2}-\frac{1}{\poly(n)}$. In fact, the $O(\log n)$ factor can be reduced to $o(\log n)$ at the price of having $\eps=\frac{1}{2}-\frac{1}{n^{o(1)}}$.} $k$-\textnormal{NCP} for $k=O(\log s)$.
\end{theorem}

The proof of this theorem is very similar \Cref{thm:w1-hardness} and \Cref{thm:gap-eth weak learning formal}. Therefore, we only include a proof sketch.

\begin{proof}[Proof sketch]
    Using \Cref{thm:general main reduction} with $\ell=2$, we reduce $O(\log n)$-approximate $k$-\textnormal{NCP} to a decision tree learning instance. In the Yes case of $O(\log n)$-approximate $k$-\textnormal{NCP}, the target will be a decision tree of size $s=2^{2k}$ which can be learned in time $n^{o(\log s)}=n^{o(k)}$. In the No case of $O(\log n)$-approximate $k$-\textnormal{NCP}, the target decision will be $(\frac{1}{2}-2^{-\Omega(k\log n)})=(\frac{1}{2}-\frac{1}{\poly(n)})$-far from every decision tree of size $2^{\Omega(k\log n)} = n^{\Omega(k)}$, and will therefore be $(\frac{1}{2}-\frac{1}{\poly(n)})$-far from the decision tree output by the learner after $n^{o(k)}$ time steps.
\end{proof}

==> feature-hardness__theorem_1_.tex <==
\subsection{Proof of \Cref{thm:NP hard intro}}
Assume there is an algorithm $\mathcal{A}$ for solving the junta testing problem described in the theorem statement. We use $\mathcal{A}$ to solve NCP. Let $(G,z)$ be an instance of $2^{\Theta(\log n/\log\log n)}$-approximate NCP with distance parameter $k$ and let $f:\zo^{2n}\to\zo$ and $\mathcal{D}$ be the function and distribution from \Cref{thm:main reduction}.  We run $\mathcal{A}$ for $t(2n)$ time steps with $r=2k$ and output ``Yes'' if and only if the algorithm outputs ``Yes''. \Cref{thm:main reduction} ensures that this reduction is efficient, as we can efficiently answer queries to $f$ and obtain random samples from $\mathcal{D}$.

\paragraph{Correctness.}{
\Cref{thm:main reduction} ensures that the reduction is correct. We expand on the Yes/No cases separately.\bigskip

\noindent
{\bf Yes case:} If $(G,z)$ is a Yes instance of $2^{\Theta(\log n/\log\log n)}$-approximate NCP, then $f$ is a $2k$-parity under $\mathcal{D}$ and $\mathcal{A}$ outputs Yes w.h.p.\bigskip

\noindent
{\bf No case:} If $(G,z)$ is a No instance of $2^{\Theta(\log n/\log\log n)}$-approximate NCP, then $f$ is $\frac{1}{2}$-far from every function of Fourier degree $k\cdot 2^{\Theta(\log n/\log\log n)}$ under $\mathcal{D}$. By the inclusion $\{k'\text{ juntas}\}\sse \{\text{degree-}k'\text{ polynomials}\}$, this implies that $f$ is $\frac{1}{2}$-far from every $k\cdot 2^{\Theta(\log n/\log\log n)}$ junta under $\mathcal{D}$. Therefore, $\mathcal{A}$ outputs No w.h.p.

}
Since $2^{\Theta(\log n/\log\log n)}$-approximate NCP is NP-hard by \Cref{thm:ncp-apx-hardness}, this reduction yields an algorithm solving SAT in $\mathrm{RTIME}(t(\poly(n)))$.\hfill\qed

==> parity-sub.tex <==
\subsection{Lifting worst-case depth to size}

In this section, we show how to lift a worst-case depth lower bound for a decision tree to a size lower bound. To do so, we use \textit{parity substitution}. The basic idea is to start with a function $f(x)$ which has large depth over a distribution $\mathcal{D}$, and substitute a parity ``block'' into each input bit of $f(x)$. This gives us a new function $f_{\oplus \ell}$ and a new distribution $\mathcal{D}_{\oplus \ell}$ with the property that if $f$ cannot be computed to error $\eps$ over $\mathcal{D}$ by depth-$d$ decision trees, then $f_{\oplus \ell}$ cannot be computed to error $\approx \eps$ over $\mathcal{D}_{\oplus \ell}$ with decision trees of size $\approx 2^d$. We formalize this transformation below.

\paragraph{Notation.}  For a string $y \in (\zo^{\ell})^n$, we write $y_i\in \zo^\ell$ to denote the $i$th block of $y$, and $(y_i)_j$ to denote the $j$th entry of the $i$th block. We define the function $\BlockwisePar: (\zo^\ell)^n \to \zo^n$: 
\[ 
\BlockwisePar(y) \coloneqq (\oplus y_1, \ldots , \oplus y_n), 
\] 
where $\oplus y_i$ denotes the parity of the bits in $y_i$. 

\begin{definition}[Parity substitution]
    For a function $f:\zo^n\to\zo$, the function $f_{\oplus \ell}:(\zo^\ell)^n$ is defined as
    $$
    f_{\oplus \ell}(y)=f(\BlockwisePar(y)).
    $$
    For a distribution $\mathcal{D}$ over $\zo^n$, the distribution $\mathcal{D}_{\oplus \ell}$ is defined via the following experiment:
    \begin{enumerate} 
    \item First sample $\bx \sim \mathcal{D}$. 
    \item For each $i\in [n]$, sample $\by_i\sim \zo^\ell$ u.a.r.~among all strings satisfying $\oplus \by_i = \bx_i$. Equivalently, sample $\by \sim (\zo^\ell)^n$ u.a.r.~among all strings satisfying $\BlockwisePar(\by) = \bx$. 
    \end{enumerate} 
\end{definition}

A key property of the distribution $\mathcal{D}_{\oplus \ell}$ is that it is ``uniform-like'' in the sense that the probability a random $\by\sim \mathcal{D}_{\oplus \ell}$ is consistent with a fixed restriction decays exponentially in the length of the restriction.

\begin{proposition}[Formal version of \Cref{prop:uniform-like-intro}]
    \label{prop:uniform-like}
    Let $R\sse [n \ell]$ be a subset of coordinates and $r\in \zo^{|R|}$. Then,
    $$
    \Prx_{\by\sim \mathcal{D}_{\oplus \ell}}[\by_R=r]\le 2^{-|R|(1-1/\ell)}.
    $$
\end{proposition}

\begin{proof}
    For $i\in [n]$, let $R_i\sse [\ell]$ denote the $i$th block of $R$, that is the subset of coordinates of the $i$th block restricted by $R$. Let $r_i$ denote the corresponding substring of $r$. We observe that
    $$
    \Prx_{\by\sim \mathcal{D}_{\oplus \ell}}[\by_{R_i}=r_i]\le\begin{cases}
        2^{-|R_i|} & |R_i|<\ell\\
        2^{-|R_i|+1} & |R_i|=\ell
    \end{cases}.
    $$
    If $|R_i|<\ell$, then the probability $\by_{R_i}=r_i$ is exactly $2^{-|R_i|}$: any subset of $\ell-1$ coordinates of the $i$th block of $\by$ is distributed uniformly at random. In the other case, $R_i$ consists of the entire $i$th block, in which case $\ell-1$ bits are distribution uniformly at random while the last bit is distributed according to $\mathcal{D}$. In either case, we can write $\Prx_{\by\sim \mathcal{D}_{\oplus \ell}}[\by_{R_i}=r_i]\le 2^{-|R_i|+|R_i|/\ell}$. Finally, we have
    \begin{align*}
        \Prx_{\by\sim \mathcal{D}_{\oplus \ell}}[\by_R=r]&=\prod_{i\in [n]}\Prx_{\by\sim \mathcal{D}_{\oplus \ell}}[\by_{R_i}=r_i]\tag{Independence of the blocks of $\by$}\\
        &\le\prod_{i\in [n]} 2^{-|R_i|+|R_i|/\ell}\\
        &=2^{-|R|(1-1/\ell)}\tag{Definition of $R_i$}
    \end{align*}
    which completes the proof. 
\end{proof}

\begin{lemma}[Pruning the depth of a decision tree]
    \label{lem:pruning-depth}
    Let $T$ be a decision tree for $f_{\oplus \ell}$ of size $s$. Let $T'$ be the decision tree obtained from $T$ by pruning each path at depth $2\log (s)$. Then $\error_{\mathcal{D}_{\oplus \ell}}(T',f_{\oplus \ell})\le\error_{\mathcal{D}_{\oplus \ell}}(T,f_{\oplus \ell})+s^{-(1-1/\ell)}$. 
\end{lemma}

\begin{proof}
    Let $P$ denote the set of paths in $T$ which have been pruned. The size of $P$ is at most $s$. By a union bound:
    \begin{align*}
        \Prx_{\by\sim \mathcal{D}_{\oplus \ell}}[T'(\by)\neq f_{\oplus \ell}(\by)]&\le \Prx_{\by \sim \mathcal{D}_{\oplus \ell}}[T(\by)\neq f_{\oplus \ell}]+\Prx_{\by \sim \mathcal{D}_{\oplus \ell}}[\by\text{ follows a path in }P]\\
        &\le \Prx_{\by \sim \mathcal{D}_{\oplus \ell}}[T(\by)\neq f_{\oplus \ell}]+\sum_{\pi \in P}\Prx_{\by \sim \mathcal{D}_{\oplus \ell}}[\by\text{ follows }\pi]\\
        &\le \Prx_{\by \sim \mathcal{D}_{\oplus \ell}}[T(\by)\neq f_{\oplus \ell}]+\sum_{\pi\in P}2^{-2\log(s)(1-1/\ell)}\tag{\Cref{prop:uniform-like} and $|\pi|\ge 2\log(s)$}\\
        &\le \Prx_{\by \sim \mathcal{D}_{\oplus \ell}}[T(\by)\neq f_{\oplus \ell}]+s^{-(1-1/\ell)}\tag{$|P|\le s$}
    \end{align*}
    which completes the proof.
\end{proof}


